HW-GPT-Bench: Hardware-Aware Architecture Benchmark for Language Models

The increasing size of language models necessitates a thorough analysis across multiple dimensions to assess trade-offs among crucial hardware metrics such as latency, energy consumption, GPU memory usage, and performance. Identifying optimal model configurations under specific hardware constraints is becoming essential but remains challenging due to the computational load of exhaustive training and evaluation on multiple devices. To address this, we introduce HW-GPT-Bench, a hardware-aware benchmark that utilizes surrogate predictions to approximate various hardware metrics across 13 devices of architectures in the GPT-2 family, with architectures containing up to 1.55B parameters. Our surrogates, via calibrated predictions and reliable uncertainty estimates, faithfully model the heteroscedastic noise inherent in the energy and latency measurements. To estimate perplexity, we employ weight-sharing techniques from Neural Architecture Search (NAS), inheriting pretrained weights from the largest GPT-2 model. Finally, we demonstrate the utility of HW-GPT-Bench by simulating optimization trajectories of various multi-objective optimization algorithms in just a few seconds.

==> 2_background.tex <==
\section{Background}
\label{sec:background}

The Transformer architecture, initially proposed by~\citet{vaswani-neurips17a}, forms the foundation of our architectural space design, with some key differences delineated in Section \ref{sec:creationofbench}. An autoregressive decoder-only transformer model has three primary building blocks: \begin{enumerate*}[label=(\roman*)]
\item \textbf{Embedding layer} to map given sentence tokens to learnable representations and encode token positions;
\item \textbf{Transformer Blocks} stacked for multiple time;
\item \textbf{Prediction Head} which predicts the next token for a given sequence.
\end{enumerate*} Furthermore, each of the transformer blocks consist of two main components \begin{enumerate*}[label=(\roman*)]\item \textbf{Causal Self Attention Block} which weighs the significance of different input tokens \item \textbf{Multi-Layer-Perceptron (MLP) block} consisting of two layers which project the input to a higher dimension and back to a lower dimension.\end{enumerate*} 

\paragraph{Architectural terminologies.} We train all our models on sequences $\mathcal{X}\in \mathcal{N}_{data}$, sampled from iid distribution $\mathcal{P}$ over vocabulary $\mathcal{V}$. The language models are trained for autoregressive language modeling tasks, where the goal is to learn a distribution over $x[t]$ token given preceding tokens $x[1:t-1]$ as context. We refer to all trainable parameters as $\theta$. Furthermore, we denote the embedding matrix as $\mathcal{W}_e \in \mathcal{R}^{d_e\times N_v}$; the positional embedding matrix as $\mathcal{W}_p \in \mathcal{R}_{d_e\times l_{max}}$. Here $d_e$ refers to the \textbf{embedding dimension}, $N_v$, the number of tokens in the vocabulary, and $l_{max}$ the maximum number of token positions in a sequence. Moreover, for the causal self-attention block, we denote the dimension of each of the query ($q$), key ($k$) and value ($v$) with $q,k,v\in \mathcal{R}^{h \times h_{dim}}$, where $h$ is the \textbf{number of heads} and $h_{dim}$, refers to the dimension of each attention head. Further for the multi-layer-perceptron (MLP) block, we define the first and second projection matrices as $\mathcal{W}_{fc_1}\in \mathcal{R}^{d_{mlp} \times d_e}$ and $\mathcal{W}_{fc_2}\in \mathcal{R}^{d_{e} \times d_{mlp}}$ respectively. Here $d_{mlp}=m*d_e$, where $m$, corresponds to the \textbf{mlp-ratio} of the MLP block. We refer to the \textbf{number of transformer blocks} in the language model as $l$. Furthermore we use $b$ to depict the \textbf{bias choice} for all linear layers in the transformer, which could be turned off or on. 

\paragraph{Search space terminologies.}  Consider a space $\mathcal{S} = \mathcal{D}_e \times \mathcal{D}_l \times \mathcal{D}_h \times \mathcal{D}_b \times \mathcal{D}_m$ of transformer architectures, where $\mathcal{D}_e$, $\mathcal{D}_l$, $\mathcal{D}_h$, $\mathcal{D}_b$ and $\mathcal{D}_m$ correspond to the set of embedding dimension choices, number of layer choices, number of head choices, choice of setting the bias in linear layers and the mlp ratio choices, respectively. Now consider a set of $m$ metrics $\mathcal{Y} = \{y_m \in \mathcal{R}^m: y = f(s), s \in \mathcal{S}\}$ eg: latency, perplexity, energy, memory consumption etc. defined for each of the architectures in the space $\mathcal{S}$. Further, assume each of the metrics in $\mathcal{Y}$ are to be minimized. We define our search space around the transformer space, with the goal of searching for different architectural modalities. Specifically we search for the optimal embedding dimension ($d_e^*$) from the set of choices $\mathcal{D}_e := \{d_{e_1}, d_{e_2}, d_{e_3}\}$, the optimal number of transformer blocks $l^*$ from $\mathcal{D}_l := \{{l_1}, {l_2}, {l_3}\}$, the optimal number of heads $h^{*}$ from $\mathcal{D}_h := \{{h_1}, {h_2}, {h_3}\}$, the choice of enabling or disabling the bias $b$ from  $\mathcal{D}_b := \{True, False\}$ and the choice of optimal mlp-ratio $m^*$ from $\mathcal{D}_m := \{m_1, m_2, m_3\}$. Furthermore, we choose the mlp-ratio and head-choice on a per-layer basis, and this amounts to a search space size of $\approx10^{36}$, at the largest scale.

\paragraph{Pareto-Front of Language Models.} 
A set of non-dominated architectures  $s^{*}$ in $\mathcal{S}$, being chosen as optimal, if no objective can be improved without sacrificing at least one other objective. On the other hand, a solution $s^{*}$ is referred to as \emph{dominated by} another solution $s$ if, and only if, $s$ is equally good or better than $s^{*}$  with respect to all objectives. Formally the \emph{Pareto-Front} of language models across different metrics in $\mathcal{Y}$ is defined as:
\begin{align*}
\mathcal{P}(\mathcal{Y}) = \{ y^{'} \in \mathcal{Y} :\{ y^{''} \in \mathcal{Y} :y^{''} < y^{'}, y^{''} \ne y^{'} \}= \emptyset \}
\end{align*}

%\paragraph{Reliable and calibrated predictions using surrogate models.}
%\todo{TODO:Lennart}
%\todo{mention other benchmarks and that they predict only one point estimate or assume gaussianity. Mention Quantile Regression, LGB, AutoGluon, etc. and the fact that they are SOTA for calibrated and accurate predictions.}

% \paragraph{Conformal Quantile Regression.}
% Quantile Regression \citep{koenker2005quantile,romano2019conformalized} models the relationship between a set of predictor (independent) variables and specific percentiles (or "quantiles") of a target (dependent) variable, most often the median. Precisely quantile regression is used when the conditions of linear regression are not satisfied i.e the dataset depicts heteroskedasticity and the errors are not normally distributed. We observe this behavior for our latency and energy observations [TODO refer to figure] and hence model distribution of latencies for an architecture using quantile regression, more specifically conformal quantile regression \citep{romano2019conformalized} to have valid coverage in finite samples, without making distributional assumptions. This gives a more realistic simulation of on-device latency and energy observations for the benchmark, contrary to other benchmarks \citep{wang2020hat}, which rely on single latency observations. 

%\todo{Add plot from utc toolbox }

==> baselines_2d_latencies_large.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_a100_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_a100_l.png}
        %\caption{Pareto Fronts and HV on A100 for GPT-L.}
        %\label{fig:baselines_latencies_a100}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_a40_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_a40_l.png}
        %\caption{Pareto Fronts and HV on A40 for GPT-L.}
        %\label{fig:baselines_latencies_a40}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_h100_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_h100_l.png}
        %\caption{Pareto Fronts and HV on H100 for GPT-L.}
        %\label{fig:baselines_latencies_h100}
    \end{minipage}
\caption{Pareto Fronts and HV on A100 (first 2), A40 (second 2) and H100 (last 2) for GPT-L}
\label{fig:baselines_latencies_a100_a40_h100}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_rtx2080_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_rtx2080_l.png}
        %\caption{Pareto Fronts and HV on RTX2080 for GPT-L.}
        %\label{fig:baselines_latencies_rtx2080}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_rtx3080_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_rtx3080_l.png}
        %\caption{Pareto Fronts and HV on RTX3080 for GPT-L.}
        %\label{fig:baselines_latencies_rtx3080}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_v100_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_v100_l.png}
        %\caption{Pareto Fronts and HV on V100 for GPT-L.}
        %\label{fig:baselines_latencies_v100}
    \end{minipage}
    \caption{Pareto Fronts and HV on RX2080 (first 2), RTX3080 (second 2) and V100 (last 2) for GPT-L}
    \label{fig:baselines_latencies_rtx2080_rtx3080_v100}
\end{figure}

\begin{figure}[ht]
\vspace{-4mm}
    \centering
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_P100_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_P100_l.png}
        %\caption{Pareto Fronts and HV on P100 for GPT-L.}
        %\label{fig:baselines_latencies_P100}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_a6000_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_a6000_l.png}
        %\caption{Pareto Fronts and HV on A6000 for GPT-L.}
        %\label{fig:baselines_latencies_a6000}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_cpu_xeon_gold_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_cpu_xeon_gold_l.png}
        %\caption{Pareto Fronts and HV on Xeon Gold for GPT-L.}
        %\label{fig:baselines_latencies_xeon_gold}
    \end{minipage}
    \caption{Pareto Fronts and HV on P100 (first 2), A6000 (second 2) and Xeon Gold CPU (last 2) for GPT-L}
    \label{fig:baselines_latencies_p100_a6000_gold}
\end{figure}
\clearpage
\begin{figure}[ht]
    \centering
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_cpu_xeon_silver_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_cpu_xeon_silver_l.png}
        %\caption{Pareto Fronts and HV on Xeon Silver for GPT-L.}
        %\label{fig:baselines_latencies_xeon_silver}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_cpu_amd_7452_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_cpu_amd_7452_l.png}
        %\caption{Pareto Fronts and HV on AMD 7452 for GPT-L.}
        %\label{fig:baselines_latencies_amd7452}
    \end{minipage}%
    \hfill
    \begin{minipage}{.33\linewidth}
        \centering
        \includegraphics[width=.49\linewidth]{hv_over_time_latencies_cpu_amd_7513_l.png}%\\[1mm]
        \includegraphics[width=.49\linewidth]{latencies_cpu_amd_7513_l.png}

        %\label{fig:baselines_latencies_amd7513}
    \end{minipage}
    \label{fig:baselines_latencies_7452_7513_silver}
        \caption{Pareto Fronts and HV on Xeon Silver (first 2), AMD 7452 (second 2) and AMD 7513 (last 2) for GPT-L}
\end{figure}


\begin{figure}[h]
\centering
\begin{minipage}{.33\textwidth}
  \centering
  \includegraphics[width=.49\linewidth]{hv_over_time_latencies_cpu_amd_7502_l.png}
\includegraphics[width=.49\linewidth]{latencies_cpu_amd_7502_l.png}
\caption{Pareto Fronts and HV on AMD 7502 for GPT-L.}
\label{fig:baselines_latencies_amd7502}
\end{minipage}
\end{figure}


==> calib_l.tex <==
\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a100_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a40_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a40_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{rtx2080_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{rtx2080_l_energies.pdf}
\end{minipage}
\caption{Prediction calibs A100, A40 and RTX280 for GPT-L}
\label{fig:calib_a100}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{rtx3080_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{rtx3080_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a6000_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{a6000_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{P100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{P100_l_energies.pdf}
\end{minipage}
\caption{Prediction calibs RTX3080, A6000, P100 for GPT-L}
\label{fig:calib_bounds_rtx3080}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{v100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{v100_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{h100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{h100_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_xeon_gold_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_xeon_gold_l_energies.pdf}
\end{minipage}
\caption{Prediction calibs V100, H100, CPU Xeon Gold for GPT-L}
\label{fig:calib_bounds_v100}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_xeon_silver_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_xeon_silver_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7452_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7452_l_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7513_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7513_l_energies.pdf}
\end{minipage}
\caption{Prediction calibs CPU Xeon Silver, AMD 7452, AMD 7513 for GPT-L}
\label{fig:calib_bounds_xeon_silver}

\end{figure}

\begin{figure}[H]
\centering
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7502_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{cpu_amd_7502_l_energies.pdf}
\end{minipage}
\caption{Prediction calibs CPU AMD 7502 for GPT-L}
\label{fig:calib_amd_7502}

\end{figure}

==> calib_tables.tex <==
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A100 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.39} & \textbf{0.03} & \textbf{0.50} & \textbf{0.28} & \textbf{0.33} & \textbf{0.02} & \textbf{0.23} & \textbf{5.68} & \textbf{1.00} & \textbf{0.17} & \textbf{1.00} & \textbf{0.42} & \textbf{0.46} & 0.09 & \textbf{0.40} & 0.08 & \textbf{0.41} & 0.08 \\ \hline
\textbf{Ensemble (XGB)} & 1.81 & 0.05 & 2.37 & 0.29 & 1.48 & 0.02 & 1.03 & 8.32 & 1.00 & 0.10 & 1.00 & 0.34 & 0.54 & \textbf{0.08} & 0.47 & 0.07 & 0.47 & 0.07 \\ \hline
\textbf{Ensemble (LGB)} & 8.74 & 0.05 & 10.14 & 0.29 & 8.37 & 0.03 & 5.06 & 9.70 & 0.97 & 0.14 & 1.00 & 0.37 & 0.57 & 0.08 & 0.49 & \textbf{0.06} & 0.49 & \textbf{0.06} \\ \hline
\textbf{Ensemble (Mix)} & 1.93 & 0.04 & 2.51 & 0.29 & 1.57 & 0.02 & 1.09 & 7.42 & 1.00 & 0.14 & 1.00 & 0.38 & 0.55 & 0.08 & 0.47 & 0.07 & 0.47 & 0.07 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa100_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A40 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.52} & \textbf{0.09} & \textbf{0.76} & \textbf{0.15} & \textbf{0.32} & \textbf{0.03} & \textbf{0.18} & \textbf{6.16} & \textbf{1.00} & \textbf{0.93} & \textbf{1.00} & \textbf{0.96} & \textbf{0.35} & 0.21 & \textbf{0.31} & 0.18 & \textbf{0.31} & 0.18 \\ \hline
\textbf{Ensemble (XGB)} & 3.16 & 0.09 & 4.19 & 0.16 & 2.43 & 0.03 & 1.26 & 6.56 & 1.00 & 0.92 & 1.00 & 0.96 & 0.54 & 0.16 & 0.46 & 0.14 & 0.47 & 0.15 \\ \hline
\textbf{Ensemble (LGB)} & 14.90 & 0.12 & 17.40 & 0.18 & 14.80 & 0.08 & 6.21 & 11.26 & 0.97 & 0.90 & 1.00 & 0.96 & 0.57 & \textbf{0.09} & 0.49 & \textbf{0.07} & 0.49 & \textbf{0.08} \\ \hline
\textbf{Ensemble (Mix)} & 3.16 & 0.09 & 4.32 & 0.15 & 2.30 & 0.03 & 1.20 & 6.49 & 1.00 & 0.93 & 1.00 & 0.96 & 0.54 & 0.17 & 0.46 & 0.15 & 0.47 & 0.15 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa40_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict H100 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.18} & \textbf{0.02} & \textbf{0.25} & \textbf{0.03} & \textbf{0.14} & \textbf{0.01} & \textbf{0.23} & \textbf{3.34} & \textbf{1.00} & \textbf{0.90} & \textbf{1.00} & \textbf{0.95} & \textbf{0.19} & \textbf{0.05} & \textbf{0.17} & \textbf{0.04} & \textbf{0.17} & \textbf{0.04} \\ \hline
\textbf{Ensemble (XGB)} & 0.76 & 0.02 & 0.99 & 0.03 & 0.61 & 0.01 & 0.98 & 3.57 & 1.00 & 0.90 & 1.00 & 0.95 & 0.48 & 0.05 & 0.41 & 0.05 & 0.42 & 0.05 \\ \hline
\textbf{Ensemble (LGB)} & 3.45 & 0.02 & 4.02 & 0.04 & 3.34 & 0.02 & 4.44 & 4.64 & 0.97 & 0.87 & 1.00 & 0.95 & 0.55 & 0.18 & 0.48 & 0.16 & 0.48 & 0.16 \\ \hline
\textbf{Ensemble (Mix)} & 0.77 & 0.02 & 1.00 & 0.03 & 0.64 & 0.01 & 0.99 & 3.50 & 1.00 & 0.90 & 1.00 & 0.95 & 0.47 & 0.05 & 0.41 & 0.05 & 0.42 & 0.05 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsh100_s}\end{table}

\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX2080 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{20.01} & \textbf{0.09} & \textbf{28.40} & \textbf{0.14} & \textbf{11.91} & \textbf{0.07} & \textbf{4.54} & \textbf{6.45} & \textbf{0.98} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.35} & 0.26 & \textbf{0.29} & 0.23 & \textbf{0.29} & 0.23 \\ \hline
\textbf{Ensemble (XGB)} & 20.59 & 0.10 & 29.58 & 0.15 & 12.17 & 0.07 & 4.60 & 6.95 & 0.97 & 0.98 & 0.99 & 0.99 & 0.42 & 0.24 & 0.35 & 0.21 & 0.36 & 0.21 \\ \hline
\textbf{Ensemble (LGB)} & 32.25 & 0.20 & 42.97 & 0.25 & 22.52 & 0.18 & 7.14 & 14.77 & 0.94 & 0.96 & 0.99 & 0.99 & 0.53 & \textbf{0.05} & 0.46 & \textbf{0.04} & 0.46 & \textbf{0.04} \\ \hline
\textbf{Ensemble (Mix)} & 20.79 & 0.10 & 29.25 & 0.15 & 13.27 & 0.08 & 4.71 & 7.52 & 0.97 & 0.98 & 0.99 & 0.99 & 0.42 & 0.21 & 0.36 & 0.19 & 0.37 & 0.20 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx2080_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX3080 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{6.21} & \textbf{0.06} & \textbf{8.83} & \textbf{0.12} & \textbf{3.69} & \textbf{0.03} & \textbf{1.97} & \textbf{4.10} & \textbf{1.00} & \textbf{0.96} & \textbf{1.00} & \textbf{0.98} & \textbf{0.43} & 0.03 & \textbf{0.36} & 0.03 & \textbf{0.37} & 0.03 \\ \hline
\textbf{Ensemble (XGB)} & 7.18 & 0.06 & 10.25 & 0.12 & 4.26 & 0.04 & 2.21 & 4.67 & 1.00 & 0.95 & 1.00 & 0.98 & 0.47 & \textbf{0.02} & 0.41 & \textbf{0.02} & 0.41 & \textbf{0.02} \\ \hline
\textbf{Ensemble (LGB)} & 22.76 & 0.10 & 27.36 & 0.16 & 21.79 & 0.08 & 7.45 & 8.40 & 0.97 & 0.92 & 1.00 & 0.98 & 0.56 & 0.25 & 0.48 & 0.22 & 0.49 & 0.23 \\ \hline
\textbf{Ensemble (Mix)} & 7.49 & 0.07 & 10.43 & 0.13 & 5.05 & 0.04 & 2.37 & 4.74 & 1.00 & 0.95 & 1.00 & 0.98 & 0.48 & 0.02 & 0.42 & 0.02 & 0.42 & 0.02 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx3080_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A6000 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1.74} & \textbf{0.05} & \textbf{2.68} & \textbf{0.06} & \textbf{1.03} & \textbf{0.04} & \textbf{0.85} & \textbf{5.95} & \textbf{1.00} & \textbf{0.93} & \textbf{1.00} & \textbf{0.96} & \textbf{0.47} & 0.04 & \textbf{0.40} & 0.03 & \textbf{0.41} & 0.03 \\ \hline
\textbf{Ensemble (XGB)} & 3.34 & 0.05 & 4.45 & 0.06 & 2.42 & 0.04 & 1.54 & 6.17 & 1.00 & 0.92 & 1.00 & 0.96 & 0.53 & \textbf{0.02} & 0.45 & \textbf{0.02} & 0.46 & \textbf{0.02} \\ \hline
\textbf{Ensemble (LGB)} & 13.46 & 0.05 & 15.83 & 0.07 & 13.16 & 0.04 & 6.48 & 6.85 & 0.97 & 0.90 & 1.00 & 0.96 & 0.57 & 0.04 & 0.49 & 0.04 & 0.49 & 0.04 \\ \hline
\textbf{Ensemble (Mix)} & 3.39 & 0.05 & 4.54 & 0.06 & 2.50 & 0.04 & 1.54 & 6.22 & 1.00 & 0.92 & 1.00 & 0.96 & 0.54 & 0.03 & 0.46 & 0.03 & 0.47 & 0.03 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa6000_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict V100 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{7.49} & \textbf{0.02} & \textbf{10.51} & \textbf{0.14} & \textbf{3.94} & \textbf{0.01} & \textbf{2.21} & \textbf{2.64} & \textbf{0.99} & \textbf{0.70} & \textbf{1.00} & \textbf{0.84} & \textbf{0.44} & \textbf{0.36} & \textbf{0.38} & \textbf{0.32} & \textbf{0.39} & \textbf{0.33} \\ \hline
\textbf{Ensemble (XGB)} & 8.03 & 0.02 & 11.42 & 0.15 & 4.60 & 0.01 & 2.41 & 3.68 & 0.99 & 0.64 & 1.00 & 0.80 & 0.47 & 0.37 & 0.41 & 0.33 & 0.41 & 0.33 \\ \hline
\textbf{Ensemble (LGB)} & 18.87 & 0.04 & 23.54 & 0.15 & 16.73 & 0.03 & 6.32 & 7.22 & 0.96 & 0.66 & 1.00 & 0.83 & 0.55 & 0.52 & 0.47 & 0.45 & 0.48 & 0.45 \\ \hline
\textbf{Ensemble (Mix)} & 8.10 & 0.02 & 11.40 & 0.14 & 4.82 & 0.01 & 2.43 & 3.40 & 0.99 & 0.69 & 1.00 & 0.83 & 0.48 & 0.37 & 0.42 & 0.32 & 0.42 & 0.33 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsv100_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict P100 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{3.62} & \textbf{0.30} & \textbf{5.31} & \textbf{0.40} & \textbf{2.36} & \textbf{0.23} & \textbf{0.21} & \textbf{6.13} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.24} & 0.26 & \textbf{0.22} & 0.23 & \textbf{0.22} & 0.23 \\ \hline
\textbf{Ensemble (XGB)} & 22.53 & 0.34 & 31.55 & 0.45 & 16.57 & 0.27 & 1.35 & 7.06 & 1.00 & 1.00 & 1.00 & 1.00 & 0.52 & 0.21 & 0.45 & 0.19 & 0.45 & 0.19 \\ \hline
\textbf{Ensemble (LGB)} & 140.75 & 0.99 & 160.96 & 1.18 & 144.00 & 1.04 & 9.42 & 22.64 & 0.97 & 0.97 & 1.00 & 1.00 & 0.57 & 0.21 & 0.49 & \textbf{0.16} & 0.49 & \textbf{0.16} \\ \hline
\textbf{Ensemble (Mix)} & 26.29 & 0.39 & 36.45 & 0.49 & 19.65 & 0.33 & 1.55 & 7.87 & 1.00 & 0.99 & 1.00 & 1.00 & 0.52 & \textbf{0.18} & 0.45 & 0.16 & 0.46 & 0.16 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsP100_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Silver latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1534.66} & \textbf{8.94} & \textbf{1982.43} & \textbf{11.88} & \textbf{1242.68} & \textbf{6.52} & \textbf{3.89} & \textbf{11.69} & \textbf{0.99} & \textbf{0.91} & \textbf{1.00} & \textbf{0.95} & \textbf{0.14} & \textbf{0.50} & \textbf{0.13} & \textbf{0.43} & \textbf{0.13} & \textbf{0.43} \\ \hline
\textbf{Ensemble (XGB)} & 1606.20 & 9.14 & 2107.51 & 12.21 & 1297.02 & 6.92 & 4.11 & 12.08 & 0.99 & 0.90 & 0.99 & 0.95 & 0.21 & 0.53 & 0.19 & 0.45 & 0.20 & 0.46 \\ \hline
\textbf{Ensemble (LGB)} & 3243.75 & 10.09 & 4020.23 & 13.66 & 2833.39 & 8.42 & 9.15 & 14.42 & 0.96 & 0.88 & 0.99 & 0.95 & 0.39 & 0.54 & 0.34 & 0.46 & 0.35 & 0.47 \\ \hline
\textbf{Ensemble (Mix)} & 1633.05 & 9.05 & 2146.05 & 12.09 & 1285.48 & 6.95 & 4.14 & 11.81 & 0.99 & 0.90 & 0.99 & 0.95 & 0.22 & 0.52 & 0.20 & 0.45 & 0.20 & 0.46 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Silver_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Gold latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1161.51} & \textbf{2.62} & \textbf{1634.77} & \textbf{3.37} & \textbf{833.97} & \textbf{2.08} & \textbf{6.49} & \textbf{9.40} & \textbf{0.96} & \textbf{0.92} & \textbf{0.98} & \textbf{0.96} & 0.12 & \textbf{0.02} & 0.10 & \textbf{0.02} & 0.10 & \textbf{0.02} \\ \hline
\textbf{Ensemble (XGB)} & 1224.12 & 2.69 & 1695.22 & 3.47 & 896.84 & 2.19 & 6.88 & 9.66 & 0.95 & 0.92 & 0.98 & 0.96 & \textbf{0.06} & 0.04 & \textbf{0.05} & 0.04 & \textbf{0.05} & 0.04 \\ \hline
\textbf{Ensemble (LGB)} & 1690.01 & 3.20 & 2144.80 & 3.98 & 1456.95 & 2.78 & 9.58 & 11.52 & 0.93 & 0.89 & 0.98 & 0.96 & 0.09 & 0.12 & 0.09 & 0.11 & 0.09 & 0.11 \\ \hline
\textbf{Ensemble (Mix)} & 1200.12 & 2.65 & 1677.90 & 3.42 & 874.13 & 2.16 & 6.68 & 9.47 & 0.95 & 0.92 & 0.98 & 0.96 & 0.07 & 0.04 & 0.06 & 0.04 & 0.06 & 0.04 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Gold_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7502 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1570.47} & \textbf{15.84} & \textbf{2297.45} & \textbf{22.15} & \textbf{1021.43} & \textbf{11.24} & \textbf{3.84} & \textbf{4.89} & \textbf{0.99} & \textbf{0.98} & \textbf{0.99} & \textbf{0.99} & \textbf{0.17} & \textbf{0.35} & \textbf{0.15} & \textbf{0.31} & \textbf{0.15} & \textbf{0.31} \\ \hline
\textbf{Ensemble (XGB)} & 1697.98 & 16.83 & 2420.66 & 23.22 & 1107.53 & 12.16 & 4.12 & 5.16 & 0.99 & 0.98 & 0.99 & 0.99 & 0.20 & 0.39 & 0.17 & 0.34 & 0.17 & 0.35 \\ \hline
\textbf{Ensemble (LGB)} & 3764.57 & 31.28 & 4531.32 & 38.53 & 3489.26 & 26.99 & 9.94 & 10.26 & 0.96 & 0.95 & 0.99 & 0.99 & 0.45 & 0.51 & 0.39 & 0.44 & 0.40 & 0.44 \\ \hline
\textbf{Ensemble (Mix)} & 1693.33 & 16.82 & 2425.90 & 23.07 & 1110.10 & 12.23 & 4.13 & 5.21 & 0.99 & 0.98 & 0.99 & 0.99 & 0.20 & 0.41 & 0.17 & 0.36 & 0.17 & 0.36 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7502_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7513 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{3321.83} & \textbf{150.24} & \textbf{5518.96} & \textbf{221.10} & \textbf{2174.08} & \textbf{103.02} & \textbf{2.76} & \textbf{10.55} & \textbf{0.99} & \textbf{0.93} & \textbf{1.00} & \textbf{0.96} & \textbf{0.38} & \textbf{0.53} & \textbf{0.34} & \textbf{0.46} & \textbf{0.34} & \textbf{0.46} \\ \hline
\textbf{Ensemble (XGB)} & 3761.37 & 157.08 & 6054.88 & 230.02 & 2633.74 & 108.79 & 3.23 & 11.14 & 0.99 & 0.92 & 1.00 & 0.96 & 0.41 & 0.54 & 0.36 & 0.46 & 0.36 & 0.47 \\ \hline
\textbf{Ensemble (LGB)} & 11204.40 & 187.74 & 13456.74 & 268.02 & 10465.21 & 150.15 & 10.68 & 14.91 & 0.96 & 0.89 & 1.00 & 0.96 & 0.55 & 0.54 & 0.47 & 0.47 & 0.48 & 0.47 \\ \hline
\textbf{Ensemble (Mix)} & 3852.39 & 154.29 & 6098.78 & 226.36 & 2635.35 & 104.72 & 3.22 & 10.85 & 0.99 & 0.92 & 1.00 & 0.96 & 0.41 & 0.54 & 0.36 & 0.47 & 0.36 & 0.47 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7513_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7452 latencies and energies on GPT-S .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{4879.20} & \textbf{14.75} & \textbf{6100.78} & \textbf{18.95} & 3820.30 & 11.39 & \textbf{9.02} & \textbf{9.21} & \textbf{0.95} & \textbf{0.95} & \textbf{0.98} & \textbf{0.97} & \textbf{0.41} & \textbf{0.47} & \textbf{0.36} & \textbf{0.41} & \textbf{0.37} & \textbf{0.41} \\ \hline
\textbf{Ensemble (XGB)} & 4930.64 & 15.06 & 6253.26 & 19.54 & 3817.53 & 11.60 & 9.16 & 9.46 & 0.95 & 0.95 & 0.98 & 0.97 & 0.44 & 0.47 & 0.39 & 0.41 & 0.39 & 0.42 \\ \hline
\textbf{Ensemble (LGB)} & 5907.72 & 18.06 & 7569.56 & 23.38 & 4669.03 & 14.40 & 11.97 & 12.29 & 0.93 & 0.92 & 0.98 & 0.97 & 0.45 & 0.48 & 0.40 & 0.41 & 0.40 & 0.42 \\ \hline
\textbf{Ensemble (Mix)} & 4903.38 & 14.94 & 6172.90 & 19.31 & \textbf{3738.50} & \textbf{11.25} & 9.12 & 9.36 & 0.95 & 0.95 & 0.98 & 0.97 & 0.46 & 0.48 & 0.40 & 0.42 & 0.40 & 0.42 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7452_s}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A100 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{2.31} & \textbf{0.10} & \textbf{3.59} & \textbf{0.36} & \textbf{1.17} & \textbf{0.06} & \textbf{0.74} & \textbf{6.50} & \textbf{1.00} & \textbf{0.84} & \textbf{1.00} & \textbf{0.92} & \textbf{0.45} & 0.40 & \textbf{0.39} & 0.35 & \textbf{0.39} & 0.36 \\ \hline
\textbf{Ensemble (XGB)} & 3.35 & 0.13 & 4.66 & 0.39 & 2.30 & 0.07 & 1.17 & 7.94 & 1.00 & 0.81 & 1.00 & 0.90 & 0.50 & 0.36 & 0.43 & 0.32 & 0.44 & 0.32 \\ \hline
\textbf{Ensemble (LGB)} & 13.88 & 0.16 & 16.12 & 0.39 & 13.82 & 0.13 & 5.37 & 12.00 & 0.97 & 0.81 & 1.00 & 0.91 & 0.57 & \textbf{0.24} & 0.49 & \textbf{0.21} & 0.49 & \textbf{0.22} \\ \hline
\textbf{Ensemble (Mix)} & 3.21 & 0.12 & 4.50 & 0.37 & 2.21 & 0.07 & 1.11 & 7.32 & 1.00 & 0.82 & 1.00 & 0.91 & 0.48 & 0.37 & 0.42 & 0.33 & 0.43 & 0.33 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa100_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A40 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1.12} & \textbf{0.26} & \textbf{1.68} & \textbf{0.35} & \textbf{0.67} & \textbf{0.18} & \textbf{0.28} & \textbf{6.38} & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & \textbf{0.99} & \textbf{0.45} & 0.20 & \textbf{0.39} & 0.18 & \textbf{0.40} & 0.18 \\ \hline
\textbf{Ensemble (XGB)} & 4.16 & 0.27 & 5.58 & 0.36 & 3.19 & 0.20 & 1.17 & 6.82 & 1.00 & 0.98 & 1.00 & 0.99 & 0.54 & 0.18 & 0.47 & 0.16 & 0.47 & 0.16 \\ \hline
\textbf{Ensemble (LGB)} & 23.39 & 0.48 & 26.62 & 0.56 & 24.93 & 0.45 & 7.11 & 13.17 & 0.97 & 0.95 & 1.00 & 0.99 & 0.57 & \textbf{0.08} & 0.49 & \textbf{0.08} & 0.49 & \textbf{0.08} \\ \hline
\textbf{Ensemble (Mix)} & 4.01 & 0.27 & 5.47 & 0.36 & 2.94 & 0.19 & 1.09 & 6.63 & 1.00 & 0.98 & 1.00 & 0.99 & 0.54 & 0.19 & 0.46 & 0.17 & 0.47 & 0.17 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa40_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict H100 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.27} & \textbf{0.05} & \textbf{0.37} & \textbf{0.07} & \textbf{0.21} & \textbf{0.04} & \textbf{0.24} & \textbf{4.57} & \textbf{1.00} & \textbf{0.95} & \textbf{1.00} & \textbf{0.98} & \textbf{0.22} & \textbf{0.24} & \textbf{0.19} & \textbf{0.21} & \textbf{0.20} & \textbf{0.21} \\ \hline
\textbf{Ensemble (XGB)} & 0.91 & 0.05 & 1.19 & 0.07 & 0.74 & 0.04 & 0.81 & 4.72 & 1.00 & 0.95 & 1.00 & 0.98 & 0.45 & 0.24 & 0.39 & 0.22 & 0.40 & 0.22 \\ \hline
\textbf{Ensemble (LGB)} & 4.49 & 0.07 & 5.14 & 0.09 & 4.54 & 0.06 & 4.04 & 6.25 & 0.97 & 0.92 & 1.00 & 0.98 & 0.56 & 0.31 & 0.48 & 0.27 & 0.48 & 0.27 \\ \hline
\textbf{Ensemble (Mix)} & 0.87 & 0.05 & 1.15 & 0.07 & 0.68 & 0.04 & 0.76 & 4.68 & 1.00 & 0.95 & 1.00 & 0.98 & 0.45 & 0.24 & 0.39 & 0.21 & 0.40 & 0.22 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsh100_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX2080 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{9.13} & \textbf{0.17} & \textbf{12.76} & \textbf{0.23} & \textbf{6.70} & \textbf{0.12} & \textbf{1.36} & \textbf{3.04} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.11} & 0.35 & \textbf{0.07} & 0.31 & \textbf{0.07} & 0.31 \\ \hline
\textbf{Ensemble (XGB)} & 11.91 & 0.19 & 16.15 & 0.27 & 8.86 & 0.14 & 1.83 & 3.35 & 0.99 & 1.00 & 1.00 & 1.00 & 0.16 & 0.32 & 0.12 & 0.28 & 0.12 & 0.29 \\ \hline
\textbf{Ensemble (LGB)} & 34.99 & 0.60 & 41.31 & 0.70 & 34.08 & 0.57 & 5.73 & 9.74 & 0.97 & 0.97 & 1.00 & 1.00 & 0.37 & \textbf{0.09} & 0.33 & \textbf{0.07} & 0.33 & \textbf{0.07} \\ \hline
\textbf{Ensemble (Mix)} & 11.58 & 0.20 & 15.82 & 0.27 & 8.78 & 0.15 & 1.76 & 3.43 & 0.99 & 1.00 & 1.00 & 1.00 & 0.16 & 0.32 & 0.12 & 0.28 & 0.13 & 0.28 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx2080_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX3080 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{2.90} & \textbf{0.82} & \textbf{4.62} & \textbf{1.06} & \textbf{1.70} & \textbf{0.59} & \textbf{0.54} & 16.97 & \textbf{1.00} & \textbf{0.93} & \textbf{1.00} & \textbf{0.97} & \textbf{0.14} & \textbf{0.20} & \textbf{0.11} & \textbf{0.18} & \textbf{0.11} & \textbf{0.19} \\ \hline
\textbf{Ensemble (XGB)} & 5.82 & 0.83 & 8.10 & 1.08 & 4.52 & 0.63 & 1.28 & 17.18 & 1.00 & 0.93 & 1.00 & 0.96 & 0.26 & 0.24 & 0.21 & 0.21 & 0.21 & 0.21 \\ \hline
\textbf{Ensemble (LGB)} & 34.62 & 1.00 & 38.99 & 1.28 & 36.60 & 0.87 & 7.87 & 22.33 & 0.97 & 0.90 & 1.00 & 0.96 & 0.55 & 0.32 & 0.47 & 0.27 & 0.48 & 0.27 \\ \hline
\textbf{Ensemble (Mix)} & 5.95 & 0.83 & 8.17 & 1.07 & 4.63 & 0.63 & 1.30 & \textbf{16.84} & 1.00 & 0.93 & 1.00 & 0.96 & 0.27 & 0.24 & 0.22 & 0.21 & 0.22 & 0.21 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx3080_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A6000 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.70} & \textbf{0.11} & \textbf{1.06} & \textbf{0.18} & \textbf{0.46} & \textbf{0.07} & \textbf{0.21} & \textbf{3.97} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.32} & 0.20 & \textbf{0.28} & 0.18 & \textbf{0.28} & 0.18 \\ \hline
\textbf{Ensemble (XGB)} & 3.66 & 0.12 & 4.93 & 0.19 & 2.82 & 0.07 & 1.16 & 4.25 & 1.00 & 0.99 & 1.00 & 0.99 & 0.52 & 0.18 & 0.45 & 0.16 & 0.46 & 0.16 \\ \hline
\textbf{Ensemble (LGB)} & 20.92 & 0.27 & 23.81 & 0.34 & 22.15 & 0.23 & 7.19 & 10.84 & 0.97 & 0.96 & 1.00 & 0.99 & 0.57 & 0.21 & 0.49 & 0.19 & 0.49 & 0.19 \\ \hline
\textbf{Ensemble (Mix)} & 3.52 & 0.14 & 4.86 & 0.20 & 2.57 & 0.10 & 1.08 & 5.25 & 1.00 & 0.99 & 1.00 & 0.99 & 0.52 & \textbf{0.10} & 0.45 & \textbf{0.09} & 0.46 & \textbf{0.09} \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa6000_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict V100 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{9.43} & \textbf{0.16} & \textbf{11.64} & \textbf{0.35} & \textbf{7.92} & \textbf{0.05} & \textbf{2.60} & \textbf{4.46} & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.37} & \textbf{0.08} & \textbf{0.33} & \textbf{0.07} & \textbf{0.33} & \textbf{0.07} \\ \hline
\textbf{Ensemble (XGB)} & 10.24 & 0.24 & 12.67 & 0.45 & 8.31 & 0.10 & 2.71 & 7.80 & 0.99 & 0.98 & 1.00 & 0.99 & 0.42 & 0.20 & 0.37 & 0.15 & 0.37 & 0.15 \\ \hline
\textbf{Ensemble (LGB)} & 26.38 & 0.54 & 30.14 & 0.67 & 25.11 & 0.42 & 6.63 & 25.46 & 0.97 & 0.96 & 1.00 & 0.99 & 0.54 & 0.40 & 0.46 & 0.34 & 0.47 & 0.35 \\ \hline
\textbf{Ensemble (Mix)} & 10.46 & 0.32 & 12.69 & 0.46 & 9.43 & 0.23 & 2.81 & 15.49 & 0.99 & 0.98 & 1.00 & 0.99 & 0.42 & 0.31 & 0.37 & 0.25 & 0.37 & 0.25 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsv100_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict P100 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{6.87} & \textbf{0.66} & \textbf{10.69} & \textbf{0.96} & \textbf{4.52} & \textbf{0.42} & \textbf{0.28} & \textbf{2.38} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.32} & 0.06 & \textbf{0.28} & 0.04 & \textbf{0.28} & 0.04 \\ \hline
\textbf{Ensemble (XGB)} & 33.86 & 0.73 & 48.02 & 1.06 & 24.22 & 0.46 & 1.39 & 2.63 & 1.00 & 1.00 & 1.00 & 1.00 & 0.52 & \textbf{0.03} & 0.45 & \textbf{0.03} & 0.46 & \textbf{0.03} \\ \hline
\textbf{Ensemble (LGB)} & 213.74 & 2.55 & 241.02 & 3.03 & 224.82 & 2.33 & 10.04 & 11.36 & 0.97 & 0.97 & 1.00 & 1.00 & 0.57 & 0.43 & 0.49 & 0.38 & 0.49 & 0.38 \\ \hline
\textbf{Ensemble (Mix)} & 38.65 & 0.89 & 52.59 & 1.21 & 28.81 & 0.69 & 1.60 & 3.61 & 1.00 & 0.99 & 1.00 & 1.00 & 0.53 & 0.08 & 0.46 & 0.06 & 0.47 & 0.07 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsP100_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Silver latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1713.09} & \textbf{13.02} & \textbf{2355.46} & \textbf{16.40} & \textbf{1261.81} & 10.12 & \textbf{3.50} & \textbf{11.85} & \textbf{0.99} & \textbf{0.94} & \textbf{1.00} & \textbf{0.97} & \textbf{0.08} & 0.54 & \textbf{0.07} & 0.46 & \textbf{0.07} & 0.47 \\ \hline
\textbf{Ensemble (XGB)} & 1867.00 & 13.19 & 2544.82 & 16.74 & 1379.22 & 10.25 & 3.78 & 12.04 & 0.99 & 0.93 & 1.00 & 0.97 & 0.14 & \textbf{0.54} & 0.12 & \textbf{0.46} & 0.12 & \textbf{0.47} \\ \hline
\textbf{Ensemble (LGB)} & 5077.16 & 15.70 & 5981.26 & 20.00 & 4830.55 & 13.47 & 10.78 & 15.19 & 0.97 & 0.91 & 1.00 & 0.97 & 0.44 & 0.54 & 0.38 & 0.46 & 0.39 & 0.47 \\ \hline
\textbf{Ensemble (Mix)} & 1913.78 & 13.05 & 2597.53 & 16.48 & 1464.40 & \textbf{9.92} & 3.87 & 11.93 & 0.99 & 0.94 & 1.00 & 0.97 & 0.14 & 0.54 & 0.12 & 0.46 & 0.12 & 0.47 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Silver_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Gold latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{997.52} & \textbf{1.78} & \textbf{1342.44} & \textbf{2.36} & \textbf{749.29} & \textbf{1.37} & \textbf{4.66} & \textbf{5.51} & \textbf{0.99} & \textbf{0.98} & \textbf{0.99} & \textbf{0.99} & 0.21 & \textbf{0.02} & 0.19 & \textbf{0.02} & 0.19 & \textbf{0.02} \\ \hline
\textbf{Ensemble (XGB)} & 1059.66 & 1.88 & 1399.18 & 2.46 & 835.65 & 1.49 & 5.00 & 5.82 & 0.99 & 0.98 & 0.99 & 0.99 & 0.19 & 0.02 & 0.17 & 0.02 & 0.17 & 0.02 \\ \hline
\textbf{Ensemble (LGB)} & 2038.55 & 3.23 & 2439.66 & 3.88 & 1886.11 & 2.99 & 9.75 & 9.79 & 0.96 & 0.96 & 0.99 & 0.99 & \textbf{0.08} & 0.22 & \textbf{0.07} & 0.20 & \textbf{0.07} & 0.20 \\ \hline
\textbf{Ensemble (Mix)} & 1042.62 & 1.88 & 1395.96 & 2.47 & 795.68 & 1.47 & 4.81 & 5.74 & 0.99 & 0.98 & 0.99 & 0.99 & 0.20 & 0.02 & 0.18 & 0.02 & 0.18 & 0.02 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Gold_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7502 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{2793.38} & \textbf{22.27} & \textbf{3832.68} & \textbf{29.64} & \textbf{2039.52} & \textbf{16.81} & \textbf{4.75} & \textbf{4.81} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.36} & \textbf{0.45} & \textbf{0.32} & \textbf{0.40} & \textbf{0.32} & \textbf{0.40} \\ \hline
\textbf{Ensemble (XGB)} & 2889.71 & 22.93 & 3927.64 & 30.61 & 2083.31 & 17.06 & 4.95 & 4.98 & 0.99 & 0.99 & 0.99 & 0.99 & 0.41 & 0.47 & 0.36 & 0.41 & 0.36 & 0.41 \\ \hline
\textbf{Ensemble (LGB)} & 5664.76 & 44.12 & 6951.41 & 54.57 & 5092.86 & 39.69 & 11.17 & 11.02 & 0.96 & 0.96 & 0.99 & 0.99 & 0.51 & 0.51 & 0.44 & 0.44 & 0.44 & 0.45 \\ \hline
\textbf{Ensemble (Mix)} & 2888.22 & 22.81 & 3930.69 & 30.58 & 2101.56 & 16.93 & 4.95 & 4.94 & 0.99 & 0.99 & 0.99 & 0.99 & 0.41 & 0.46 & 0.36 & 0.40 & 0.36 & 0.40 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7502_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7513 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{3297.57} & \textbf{315.32} & \textbf{6512.33} & \textbf{708.51} & \textbf{1709.93} & \textbf{174.70} & \textbf{1.92} & \textbf{14.36} & \textbf{1.00} & \textbf{0.74} & \textbf{1.00} & \textbf{0.86} & \textbf{0.46} & 0.55 & \textbf{0.40} & 0.48 & \textbf{0.40} & 0.48 \\ \hline
\textbf{Ensemble (XGB)} & 4020.05 & 344.26 & 7071.85 & 724.33 & 2639.66 & 200.98 & 2.55 & 15.96 & 1.00 & 0.72 & 1.00 & 0.85 & 0.49 & 0.55 & 0.43 & 0.48 & 0.43 & 0.48 \\ \hline
\textbf{Ensemble (LGB)} & 15744.34 & 367.84 & 18417.64 & 744.75 & 15733.28 & 256.65 & 11.25 & 19.37 & 0.97 & 0.71 & 1.00 & 0.85 & 0.57 & 0.56 & 0.49 & 0.48 & 0.49 & 0.49 \\ \hline
\textbf{Ensemble (Mix)} & 4390.21 & 329.13 & 7277.61 & 717.62 & 3043.23 & 183.58 & 2.72 & 14.82 & 0.99 & 0.73 & 1.00 & 0.85 & 0.50 & \textbf{0.55} & 0.44 & \textbf{0.48} & 0.44 & \textbf{0.48} \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7513_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7452 latencies and energies on GPT-M .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{6422.40} & \textbf{19.16} & \textbf{8400.06} & \textbf{25.91} & \textbf{4603.69} & \textbf{13.53} & \textbf{8.76} & \textbf{8.80} & \textbf{0.96} & \textbf{0.96} & \textbf{0.98} & \textbf{0.98} & \textbf{0.40} & \textbf{0.43} & \textbf{0.34} & \textbf{0.37} & \textbf{0.35} & \textbf{0.38} \\ \hline
\textbf{Ensemble (XGB)} & 6583.99 & 19.77 & 8650.39 & 26.64 & 4800.54 & 14.12 & 9.01 & 9.17 & 0.96 & 0.96 & 0.98 & 0.98 & 0.46 & 0.47 & 0.40 & 0.41 & 0.41 & 0.42 \\ \hline
\textbf{Ensemble (LGB)} & 8414.41 & 25.28 & 11082.78 & 33.29 & 6746.91 & 20.86 & 13.18 & 13.17 & 0.93 & 0.93 & 0.98 & 0.98 & 0.49 & 0.51 & 0.43 & 0.44 & 0.43 & 0.44 \\ \hline
\textbf{Ensemble (Mix)} & 6535.60 & 19.66 & 8556.66 & 26.48 & 5013.65 & 14.41 & 8.93 & 9.06 & 0.96 & 0.96 & 0.98 & 0.98 & 0.46 & 0.47 & 0.40 & 0.41 & 0.40 & 0.41 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7452_m}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A100 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1.43} & \textbf{0.34} & \textbf{1.97} & \textbf{0.56} & \textbf{1.14} & \textbf{0.16} & \textbf{0.70} & \textbf{6.63} & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & \textbf{0.99} & 0.31 & 0.39 & 0.24 & 0.34 & 0.24 & 0.34 \\ \hline
\textbf{Ensemble (XGB)} & 2.07 & 0.36 & 2.85 & 0.58 & 1.55 & 0.18 & 1.00 & 7.55 & 1.00 & 0.97 & 1.00 & 0.99 & 0.30 & 0.35 & 0.22 & 0.31 & 0.23 & 0.32 \\ \hline
\textbf{Ensemble (LGB)} & 9.28 & 0.67 & 10.63 & 0.84 & 9.24 & 0.54 & 4.75 & 18.27 & 0.97 & 0.95 & 1.00 & 0.99 & 0.46 & \textbf{0.13} & 0.41 & \textbf{0.10} & 0.41 & \textbf{0.10} \\ \hline
\textbf{Ensemble (Mix)} & 2.16 & 0.38 & 2.94 & 0.58 & 1.68 & 0.21 & 1.04 & 8.26 & 1.00 & 0.97 & 1.00 & 0.99 & \textbf{0.29} & 0.34 & \textbf{0.22} & 0.30 & \textbf{0.22} & 0.31 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa100_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A40 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.61} & \textbf{0.18} & \textbf{0.90} & \textbf{0.23} & \textbf{0.41} & \textbf{0.15} & \textbf{0.27} & \textbf{2.43} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.44} & 0.38 & \textbf{0.39} & 0.34 & \textbf{0.39} & 0.35 \\ \hline
\textbf{Ensemble (XGB)} & 2.44 & 0.23 & 3.37 & 0.28 & 1.81 & 0.19 & 1.11 & 2.88 & 1.00 & 1.00 & 1.00 & 1.00 & 0.54 & 0.36 & 0.47 & 0.32 & 0.47 & 0.32 \\ \hline
\textbf{Ensemble (LGB)} & 15.23 & 0.83 & 17.17 & 0.95 & 16.50 & 0.87 & 7.69 & 10.53 & 0.97 & 0.97 & 1.00 & 1.00 & 0.57 & \textbf{0.06} & 0.49 & \textbf{0.05} & 0.49 & \textbf{0.05} \\ \hline
\textbf{Ensemble (Mix)} & 2.41 & 0.22 & 3.34 & 0.28 & 1.74 & 0.19 & 1.07 & 2.79 & 1.00 & 1.00 & 1.00 & 1.00 & 0.54 & 0.36 & 0.47 & 0.32 & 0.47 & 0.33 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa40_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict H100 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{0.15} & \textbf{0.13} & \textbf{0.21} & \textbf{0.17} & \textbf{0.11} & 0.09 & \textbf{0.15} & \textbf{5.37} & \textbf{1.00} & \textbf{0.96} & \textbf{1.00} & \textbf{0.98} & \textbf{0.22} & 0.16 & \textbf{0.20} & 0.14 & \textbf{0.20} & 0.14 \\ \hline
\textbf{Ensemble (XGB)} & 0.62 & 0.13 & 0.83 & 0.18 & 0.47 & 0.09 & 0.63 & 5.50 & 1.00 & 0.96 & 1.00 & 0.98 & 0.48 & 0.16 & 0.42 & 0.14 & 0.42 & 0.14 \\ \hline
\textbf{Ensemble (LGB)} & 3.61 & 0.18 & 4.11 & 0.23 & 3.79 & 0.15 & 3.84 & 8.09 & 0.97 & 0.93 & 1.00 & 0.98 & 0.56 & 0.27 & 0.48 & 0.25 & 0.49 & 0.25 \\ \hline
\textbf{Ensemble (Mix)} & 0.57 & 0.13 & 0.78 & 0.17 & 0.41 & \textbf{0.08} & 0.57 & 5.41 & 1.00 & 0.96 & 1.00 & 0.98 & 0.47 & \textbf{0.16} & 0.41 & \textbf{0.14} & 0.41 & \textbf{0.14} \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsh100_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX2080 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{2.40} & \textbf{1.80} & \textbf{3.43} & \textbf{2.58} & \textbf{1.53} & 1.12 & \textbf{0.59} & \textbf{10.68} & \textbf{1.00} & \textbf{0.90} & \textbf{1.00} & \textbf{0.95} & 0.16 & \textbf{0.24} & 0.14 & \textbf{0.22} & 0.14 & \textbf{0.22} \\ \hline
\textbf{Ensemble (XGB)} & 5.21 & 1.83 & 6.98 & 2.63 & 4.06 & 1.15 & 1.30 & 10.91 & 1.00 & 0.90 & 1.00 & 0.95 & \textbf{0.16} & 0.29 & \textbf{0.13} & 0.25 & \textbf{0.13} & 0.25 \\ \hline
\textbf{Ensemble (LGB)} & 28.00 & 2.09 & 31.84 & 2.92 & 30.68 & 1.42 & 7.61 & 13.14 & 0.97 & 0.88 & 1.00 & 0.95 & 0.35 & 0.35 & 0.32 & 0.30 & 0.32 & 0.31 \\ \hline
\textbf{Ensemble (Mix)} & 4.79 & 1.83 & 6.60 & 2.62 & 3.46 & \textbf{1.09} & 1.14 & 10.92 & 1.00 & 0.90 & 1.00 & 0.95 & 0.16 & 0.30 & 0.13 & 0.26 & 0.13 & 0.27 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx2080_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict RTX3080 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1.49} & \textbf{0.68} & \textbf{2.13} & \textbf{0.77} & \textbf{0.99} & 0.66 & \textbf{0.50} & \textbf{6.50} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & \textbf{0.13} & 0.07 & \textbf{0.12} & 0.06 & \textbf{0.12} & 0.06 \\ \hline
\textbf{Ensemble (XGB)} & 3.95 & 0.70 & 5.40 & 0.81 & 2.89 & 0.65 & 1.36 & 6.59 & 1.00 & 0.99 & 1.00 & 1.00 & 0.21 & 0.07 & 0.15 & 0.06 & 0.16 & 0.06 \\ \hline
\textbf{Ensemble (LGB)} & 22.68 & 1.46 & 25.65 & 1.71 & 24.92 & 1.42 & 8.86 & 12.08 & 0.97 & 0.96 & 1.00 & 1.00 & 0.52 & 0.12 & 0.45 & 0.11 & 0.46 & 0.11 \\ \hline
\textbf{Ensemble (Mix)} & 3.86 & 0.69 & 5.32 & 0.81 & 2.78 & \textbf{0.65} & 1.32 & 6.56 & 1.00 & 0.99 & 1.00 & 1.00 & 0.23 & \textbf{0.07} & 0.17 & \textbf{0.06} & 0.17 & \textbf{0.06} \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsrtx3080_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict A6000 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1.56} & \textbf{0.45} & \textbf{2.24} & \textbf{0.61} & \textbf{1.08} & \textbf{0.33} & \textbf{0.74} & \textbf{7.13} & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & \textbf{0.99} & \textbf{0.48} & 0.20 & \textbf{0.42} & 0.17 & \textbf{0.42} & 0.18 \\ \hline
\textbf{Ensemble (XGB)} & 2.22 & 0.47 & 3.06 & 0.63 & 1.57 & 0.34 & 1.11 & 7.21 & 1.00 & 0.98 & 1.00 & 0.99 & 0.51 & 0.19 & 0.44 & 0.17 & 0.45 & 0.17 \\ \hline
\textbf{Ensemble (LGB)} & 13.40 & 0.84 & 15.18 & 1.04 & 14.58 & 0.67 & 7.47 & 12.16 & 0.97 & 0.95 & 1.00 & 0.99 & 0.57 & \textbf{0.03} & 0.49 & \textbf{0.02} & 0.49 & \textbf{0.02} \\ \hline
\textbf{Ensemble (Mix)} & 2.08 & 0.46 & 2.95 & 0.63 & 1.45 & 0.34 & 0.99 & 7.36 & 1.00 & 0.98 & 1.00 & 0.99 & 0.50 & 0.17 & 0.43 & 0.15 & 0.44 & 0.15 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsa6000_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict V100 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & 11.61 & \textbf{0.30} & \textbf{13.29} & \textbf{2.99} & 11.30 & \textbf{0.15} & 4.23 & \textbf{3.74} & \textbf{0.98} & \textbf{0.86} & \textbf{0.99} & \textbf{0.93} & \textbf{0.52} & 0.21 & \textbf{0.45} & 0.19 & \textbf{0.45} & 0.19 \\ \hline
\textbf{Ensemble (XGB)} & \textbf{11.50} & 0.44 & 13.66 & 3.02 & \textbf{10.46} & 0.25 & \textbf{4.16} & 6.43 & 0.98 & 0.86 & 0.99 & 0.93 & 0.54 & \textbf{0.05} & 0.47 & \textbf{0.05} & 0.47 & \textbf{0.05} \\ \hline
\textbf{Ensemble (LGB)} & 17.77 & 1.32 & 22.53 & 3.31 & 13.23 & 1.34 & 6.55 & 25.45 & 0.96 & 0.83 & 0.99 & 0.93 & 0.54 & 0.34 & 0.46 & 0.30 & 0.47 & 0.30 \\ \hline
\textbf{Ensemble (Mix)} & 11.84 & 0.43 & 13.63 & 3.03 & 10.69 & 0.24 & 4.35 & 6.30 & 0.98 & 0.86 & 0.99 & 0.93 & 0.55 & 0.07 & 0.47 & 0.06 & 0.48 & 0.06 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsv100_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict P100 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{5.59} & \textbf{0.78} & \textbf{7.81} & \textbf{1.27} & \textbf{4.28} & \textbf{0.40} & \textbf{0.52} & \textbf{1.31} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.29} & 0.13 & \textbf{0.26} & 0.11 & \textbf{0.26} & 0.12 \\ \hline
\textbf{Ensemble (XGB)} & 21.84 & 1.17 & 29.68 & 1.77 & 16.52 & 0.73 & 1.61 & 2.18 & 1.00 & 1.00 & 1.00 & 1.00 & 0.49 & \textbf{0.06} & 0.43 & \textbf{0.06} & 0.43 & \textbf{0.06} \\ \hline
\textbf{Ensemble (LGB)} & 131.33 & 5.74 & 146.45 & 6.60 & 139.03 & 5.69 & 10.74 & 13.53 & 0.97 & 0.97 & 1.00 & 1.00 & 0.57 & 0.50 & 0.49 & 0.44 & 0.49 & 0.44 \\ \hline
\textbf{Ensemble (Mix)} & 23.97 & 1.64 & 31.74 & 2.20 & 18.94 & 1.30 & 1.76 & 3.66 & 1.00 & 1.00 & 1.00 & 1.00 & 0.49 & 0.20 & 0.42 & 0.18 & 0.43 & 0.18 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsP100_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Silver latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{636.15} & 5.61 & \textbf{864.06} & \textbf{7.70} & \textbf{494.13} & 3.93 & \textbf{2.54} & \textbf{9.84} & \textbf{1.00} & \textbf{0.96} & \textbf{1.00} & \textbf{0.98} & 0.17 & 0.44 & 0.15 & 0.38 & 0.15 & 0.39 \\ \hline
\textbf{Ensemble (XGB)} & 753.47 & 5.72 & 1025.05 & 7.81 & 578.99 & 4.01 & 2.96 & 10.02 & 1.00 & 0.96 & 1.00 & 0.98 & 0.08 & \textbf{0.42} & 0.07 & \textbf{0.36} & 0.07 & \textbf{0.37} \\ \hline
\textbf{Ensemble (LGB)} & 2824.18 & 8.02 & 3236.41 & 9.97 & 2733.85 & 6.99 & 11.64 & 14.87 & 0.97 & 0.93 & 1.00 & 0.98 & 0.41 & 0.48 & 0.37 & 0.41 & 0.37 & 0.42 \\ \hline
\textbf{Ensemble (Mix)} & 794.59 & \textbf{5.60} & 1061.38 & 7.73 & 619.52 & \textbf{3.82} & 3.12 & 10.00 & 1.00 & 0.96 & 1.00 & 0.98 & \textbf{0.06} & 0.42 & \textbf{0.05} & 0.36 & \textbf{0.06} & 0.37 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Silver_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict Xeon Gold latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1808.83} & \textbf{2.94} & \textbf{4993.72} & \textbf{9.06} & \textbf{961.39} & \textbf{1.64} & \textbf{12.44} & \textbf{12.52} & \textbf{0.65} & \textbf{0.60} & \textbf{0.81} & \textbf{0.77} & \textbf{0.04} & \textbf{0.22} & \textbf{0.03} & \textbf{0.20} & \textbf{0.03} & \textbf{0.20} \\ \hline
\textbf{Ensemble (XGB)} & 2071.91 & 3.33 & 5172.30 & 9.21 & 1192.99 & 2.01 & 14.28 & 14.39 & 0.62 & 0.58 & 0.79 & 0.76 & 0.23 & 0.36 & 0.21 & 0.32 & 0.21 & 0.32 \\ \hline
\textbf{Ensemble (LGB)} & 2276.83 & 3.72 & 5208.21 & 9.42 & 1546.31 & 2.52 & 16.82 & 17.10 & 0.62 & 0.56 & 0.80 & 0.76 & 0.32 & 0.42 & 0.28 & 0.37 & 0.28 & 0.37 \\ \hline
\textbf{Ensemble (Mix)} & 1956.75 & 3.15 & 5056.95 & 9.17 & 1058.07 & 1.74 & 13.15 & 13.29 & 0.64 & 0.59 & 0.80 & 0.77 & 0.21 & 0.35 & 0.18 & 0.31 & 0.18 & 0.31 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsXeon Gold_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7502 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{979.59} & \textbf{10.85} & \textbf{1401.41} & \textbf{15.13} & \textbf{637.77} & \textbf{7.47} & \textbf{3.47} & \textbf{4.78} & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.32} & 0.46 & \textbf{0.29} & 0.40 & \textbf{0.29} & 0.41 \\ \hline
\textbf{Ensemble (XGB)} & 1061.60 & 11.30 & 1488.69 & 15.60 & 747.04 & 8.16 & 3.90 & 5.16 & 0.99 & 0.99 & 1.00 & 0.99 & 0.36 & 0.47 & 0.32 & 0.41 & 0.32 & 0.41 \\ \hline
\textbf{Ensemble (LGB)} & 2963.13 & 24.72 & 3487.50 & 29.94 & 2788.52 & 22.54 & 12.75 & 13.26 & 0.96 & 0.96 & 1.00 & 0.99 & 0.53 & 0.54 & 0.46 & 0.47 & 0.46 & 0.47 \\ \hline
\textbf{Ensemble (Mix)} & 1077.05 & 11.22 & 1504.92 & 15.53 & 777.37 & 8.19 & 3.88 & 4.97 & 0.99 & 0.99 & 1.00 & 0.99 & 0.34 & \textbf{0.44} & 0.30 & \textbf{0.38} & 0.31 & \textbf{0.39} \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7502_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7513 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{1341.23} & \textbf{138.82} & \textbf{2336.42} & \textbf{193.98} & \textbf{747.38} & \textbf{92.12} & \textbf{1.55} & \textbf{13.84} & \textbf{1.00} & \textbf{0.91} & \textbf{1.00} & \textbf{0.96} & \textbf{0.48} & \textbf{0.55} & \textbf{0.42} & \textbf{0.48} & \textbf{0.42} & \textbf{0.48} \\ \hline
\textbf{Ensemble (XGB)} & 1821.68 & 141.56 & 2867.87 & 198.08 & 1203.03 & 97.95 & 2.32 & 14.26 & 1.00 & 0.91 & 1.00 & 0.95 & 0.53 & 0.56 & 0.45 & 0.48 & 0.46 & 0.48 \\ \hline
\textbf{Ensemble (LGB)} & 8438.54 & 158.86 & 9602.56 & 224.77 & 8622.26 & 129.98 & 12.73 & 18.19 & 0.97 & 0.88 & 1.00 & 0.95 & 0.57 & 0.56 & 0.49 & 0.48 & 0.49 & 0.49 \\ \hline
\textbf{Ensemble (Mix)} & 1990.32 & 141.12 & 2967.07 & 197.03 & 1402.25 & 103.07 & 2.56 & 14.02 & 1.00 & 0.91 & 1.00 & 0.95 & 0.53 & 0.56 & 0.46 & 0.48 & 0.46 & 0.49 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7513_l}\end{table}
\begin{table}[ht]\centering\caption{Various performance metrics of surrogates evaluated to predict AMD 7452 latencies and energies on GPT-L .The arrow on the side of the metric name indicates if lower or higher is better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclclclclclclclclclcl} 
\toprule
\multirow{2}{*}{\textbf{Surrogate}} & \multicolumn{12}{c}{\textbf{Accuracy}}                                                                                                                                                                                                                                                                                                   & \multicolumn{6}{c}{\textbf{Calibration}}                                                                                                                      \\ 
\cmidrule(lr){2-13}\cmidrule(lr){14-19}
                                    & \multicolumn{2}{c}{\textbf{MAE} $\downarrow$}                   & \multicolumn{2}{c}{\textbf{RMSE} $\downarrow$}                               & \multicolumn{2}{c}{\textbf{MDAE} $\downarrow$}                  & \multicolumn{2}{c}{\textbf{MARPD} $\downarrow$}                 & \multicolumn{2}{c}{\textbf{R\textsuperscript{2}} $\uparrow$}  & \multicolumn{2}{c}{\textbf{Corr.} $\uparrow$}                  & \multicolumn{2}{c}{\textbf{RMS Cal.} $\downarrow$}               & \multicolumn{2}{c}{\textbf{MA Cal.} $\downarrow$}                & \multicolumn{2}{c}{\textbf{Miscal. Area} $\downarrow$}            \\ 
\midrule
\multicolumn{1}{c}{}                & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}               & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}} & \textbf{latencies}  & \multicolumn{1}{c}{\textbf{energies}}  \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15} \cmidrule(lr){16-17}\cmidrule(lr){18-19}
\textbf{AutoGluon} & \textbf{766.81} & \textbf{4.16} & \textbf{1101.54} & \textbf{6.15} & \textbf{535.75} & \textbf{2.72} & \textbf{2.52} & \textbf{4.20} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & \textbf{0.05} & \textbf{0.26} & \textbf{0.04} & \textbf{0.23} & \textbf{0.05} & \textbf{0.23} \\ \hline
\textbf{Ensemble (XGB)} & 895.53 & 4.40 & 1262.25 & 6.44 & 636.53 & 3.02 & 2.98 & 4.55 & 1.00 & 0.99 & 1.00 & 1.00 & 0.14 & 0.29 & 0.12 & 0.26 & 0.13 & 0.26 \\ \hline
\textbf{Ensemble (LGB)} & 3265.62 & 10.37 & 3747.71 & 12.55 & 3294.40 & 9.69 & 12.28 & 12.92 & 0.97 & 0.96 & 1.00 & 0.99 & 0.50 & 0.50 & 0.43 & 0.43 & 0.44 & 0.44 \\ \hline
\textbf{Ensemble (Mix)} & 920.19 & 4.45 & 1277.03 & 6.47 & 681.07 & 2.98 & 3.07 & 4.57 & 1.00 & 0.99 & 1.00 & 0.99 & 0.14 & 0.29 & 0.13 & 0.26 & 0.13 & 0.26 \\ \hline
\bottomrule
\end{tabular}
}
\vspace{-3ex}\label{tab:surrogatemetricsAMD 7452_l}\end{table}


==> confidence_plots.tex <==

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a100_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds A100}
\label{fig:confidence_bounds_a100}

\end{figure}
\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a40_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds A40}
\label{fig:confidence_bounds_a40}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx2080_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds RTX2080}
\label{fig:confidence_bounds_rtx2080}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/rtx3080_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds RTX3080}
\label{fig:confidence_bounds_rtx3080}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/a6000_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds A6000}
\label{fig:confidence_bounds_a6000}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/P100_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds P100}
\label{fig:confidence_bounds_p100}

\end{figure}

\begin{figure}[H]

\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/v100_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds V100}
\label{fig:confidence_bounds_v100}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/h100_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds H100}
\label{fig:confidence_bounds_h100}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_gold_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds Xeon Gold}
\label{fig:confidence_bounds_xeon_gold}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_xeon_silver_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds Xeon Silver}
\label{fig:confidence_bounds_xeon_silver}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7452_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds CPU AMD 7452}
\label{fig:confidence_amd_7452}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7513_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds CPU AMD 7513}
\label{fig:confidence_amd_7513}

\end{figure}

\begin{figure}[H]
\begin{minipage}{.16\linewidth}
  \centering
  \includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_s_latencies.pdf}
\end{minipage}%
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_s_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_m_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_m_energies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_l_latencies.pdf}
\end{minipage}
\begin{minipage}{.16\linewidth}
  \centering
\includegraphics[width=\linewidth]{neurips_dbt/confidence_plots/cpu_amd_7502_l_energies.pdf}
\end{minipage}
\caption{Confidence Bounds CPU AMD 7502}
\label{fig:confidence_amd_7502}

\end{figure}

==> impact.tex <==
\section*{Broader Impact and Societal Implications}

With HW-GPT-Bench, we hope to provide a significant contribution to the field of hardware-aware architecture search and structural pruning for large language models (LLMs). By enabling efficient exploration of Pareto-optimal configurations across multiple hardware metrics, our work has several broader impacts and societal implications:

\begin{itemize}[leftmargin=*]
    \item \textbf{Energy Efficiency and Environmental Impact.} The increasing computational demands of training and deploying LLMs contribute significantly to global energy consumption. HW-GPT-Bench aims to optimize LLM configurations to reduce energy usage, thereby mitigating the environmental impact associated with large-scale AI deployments. By identifying energy-efficient architectures, our benchmark supports the development of sustainable AI technologies.
    \item \textbf{Enhanced Research and Development.} HW-GPT-Bench facilitates the rapid prototyping and evaluation of new multi-objective optimization algorithms. By providing a comprehensive benchmark, it accelerates research in the field of neural architecture search (NAS) and structural pruning. This can lead to the discovery of architectures that have better energy-performance tradeoffs.
    \item \textbf{Accessibility and Democratization of AI.} Efficient LLMs that perform well across various hardware configurations make advanced AI capabilities more accessible to a wider range of users and organizations, particularly those with limited computational resources. This democratization of AI technology can drive innovation and enable smaller entities to leverage state-of-the-art language models for diverse applications.
    \item \textbf{Economic Benefits.} Optimizing for hardware efficiency can lead to substantial cost savings in both the training and deployment phases of LLMs. By reducing the computational resources required, organizations can achieve economic benefits, making it more feasible to deploy AI solutions at scale. This economic efficiency is particularly beneficial for industries reliant on large-scale data processing and analysis.
    \item \textbf{Ethical AI Deployment.} The ability to optimize models for specific hardware and efficiency metrics can support more ethical AI deployment practices. For example, reducing latency and energy consumption can enhance user experience and accessibility, while also ensuring that the deployment of AI systems is more environmentally responsible.
\end{itemize}

Overall, the HW-GPT-Bench framework addresses critical challenges in the development and deployment of algorithms that search on LLM spaces, eventually promoting a more sustainable, accessible, and economically viable AI ecosystem. It underscores the importance of considering hardware efficiency alongside performance in the advancement of AI technologies.
